A Unified Encoder-Decoder Framework with Entity Memory

Entities, as important carriers of real-world knowledge, play a key role in many NLP tasks. We focus on incorporating entity knowledge into an encoder-decoder framework for informative text generation. Existing approaches tried to index, retrieve, and read external documents as evidence, but they suffered from a large computational overhead. In this work, we propose an encoder-decoder framework with an entity memory, namely EDMem. The entity knowledge is stored in the memory as latent representations, and the memory is pre-trained on Wikipedia along with encoder-decoder parameters. To precisely generate entity names, we design three decoding methods to constrain entity generation by linking entities in the memory. EDMem is a unified framework that can be used on various entity-intensive question answering and generation tasks. Extensive experimental results show that EDMem outperforms both memory-based auto-encoder models and non-memory encoder-decoder models.

==> figures/figure-analysis.tex <==
\begin{figure*}[t]
% \centering
\begin{minipage}[t]{0.3\textwidth}
% \centering
\includegraphics[width=4.75cm]{figures/memory_size.pdf}
\vspace{-0.5cm}
\setcaptionwidth{0.9\textwidth}
\caption{Effect of different memory sizes on performances of EDMem and EncMem on TQA.}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
% \centering
\includegraphics[width=4.75cm]{figures/memory_size_linkable.pdf}
\vspace{-0.5cm}
\setcaptionwidth{0.9\textwidth}
\caption{Effect of different memory sizes on EDMem's performance on linkable and non-linkable answers of TQA}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
% \centering
\includegraphics[width=4.75cm]{figures/training_step.pdf}
\vspace{-0.5cm}
\setcaptionwidth{0.9\textwidth}
\caption{TQA performance on different number of pre-training steps.}
\end{minipage}
\end{figure*}


==> figures/figure-finetune.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.7]{figures/Fine-tune.pdf}
    \caption{Three decoding methods used in down-stream fine-tuning. \cz{from this figure alone, it's very hard to tell the difference between static and dynamic linking.}}
    \label{fig:finetune}
    \vspace{-0.75cm}
\end{figure}

==> figures/figure-trie.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.55]{figures/Trie.pdf}
    \vspace{-0.25cm}
    \caption{An example of a prefix tree for entities ``United States'', ``United Kingdom'' and ``Ireland''. If the model already generated ``$[E_s]$ United'', the only valid tokens next are ``States'' and ``Kingdom''.}
    \label{fig:trie}
    \vspace{-0.5cm}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/table-OpenQA-demo.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.5mm}{
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{TQA}} & \textbf{NQ}    & \textbf{WQ}    \\
                                & In-House Test & Dev   & Test           & Test           \\ \midrule
\multicolumn{5}{c}{\textit{Closed-Book Models}}                                                      \\ \midrule
BART-Large*                      & 25.02           & 27.28           & 24.82          & 29.23          \\
% T5-Large*                   & -           &   28.70             & 28.50          & 30.60          \\
EncDec*   & 27.54 & 30.01  & 25.96 & 29.38 \\
% RELIC\dag                           & 35.70           & -              & -              & -              \\
EaE\dag                             & -               & 43.20          & -              & 39.00    \\
% FILM\dag                            & 29.10           & -              & -              & -              \\
EncMem\dag                  & 41.01             & 42.00         & 25.54                 & 38.88   \\
EDMem-free               & 42.24           & 43.31          & {\underline{29.14}}    & 36.47          \\
EDMem-static              & \textbf{46.19}  & \textbf{47.23} & \textbf{30.19} & \textbf{41.44} \\
EDMem-dynamic        & {\underline{43.82}}     & {\underline{44.44}}    & 27.70          & \underline{39.52}          \\ \midrule
\multicolumn{5}{c}{\textit{Open-Book SOTA}}                                                        \\ \midrule
% REALM                           & -               & -              & 40.40          & 40.70          \\
% DPR+BERT                        & \textbf{56.80}  & -              & 41.50          & 42.40          \\
% RAG                             & 56.80  & -              & 44.50 & 45.20 \\
FiD                             & 67.60  & -              & 51.40 & 47.64 \\\bottomrule
\end{tabular}}}
\caption{Exact match scores on open-domain QA datasets. \textbf{Bold} scores and \underline{underlined} scores are the best and second best results among closed-book models. (*traditional encoder-decoder models, \dag memory-based auto-encoder models)}
% \vspace{-0.25cm}
\end{table}

==> tables/table-contribution.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{1.3mm}{
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
Models & Knowledge & Generation & Efficiency \\
\midrule
Encoder+Decoder  & Parameters         & \cmark          & Good       \\
Encoder+Memory   & Memory         & \xmark          & Good       \\
Open-Book   & Documents         & \cmark          & Bad        \\
EDMem (Ours)  & Memory         & \cmark          & Good      \\ \bottomrule
\end{tabular}}}
\caption{Comparison between different models.}
\label{tab:contrib}
\vspace{-0.5cm}
\end{table}

==> tables/table-generation-demo.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|lcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}}                                                            & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ROUGE-L}} & \multirow{2}{*}{\textbf{F1}}  & \multicolumn{2}{c}{\textbf{Entity Coverage}} \\
&&&& Total & Unseen \\ \midrule
\multirow{3}{*}{MSMARCO}                                                     & BART-Large                 & 53.26            & 53.86   & 43.87              & 22.40                     \\
                                                                             & EDMem-free              & \textbf{54.45}            & \textbf{55.08}       & 45.53              & 25.33                     \\
                                                                             & EDMem-dyn.     & 52.84            & 52.94       & \textbf{51.28}              & \textbf{28.49}                    \\\cmidrule{1-6}
                                                                            %  & FiD (open-book)  &     60.54        &     42.96        &     57.22        &  58.12   &  79.79   &   49.63           &     32.58               \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}CREAK\\\end{tabular}} & BART-Large                & 30.34            &      30.20     & 46.87              & 14.98                     \\
                                                                             & EDMem-free            & \textbf{31.78}            &    \textbf{31.34}       & 49.06              & 16.65                     \\
                                                                             & EDMem-dyn.              & 30.68            &       30.32       & \textbf{49.90}              & \textbf{18.76}                     \\\cmidrule{1-6}
                                                                            %  & FiD (open-book)  &      35.96       &     18.11        &      33.54       &  33.57   &   81.02  &     51.02           &        21.09              \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ELI5\end{tabular}}      & BART-Large                  & 22.99            &      19.38     & 29.18              & 14.83                     \\
                                                                             & EDMem-free              & 23.24            &     20.19        & 38.76              & 18.61                    \\
                                                                             & EDMem-dyn.      & \textbf{23.97}            &      \textbf{20.66}     & \textbf{45.66}              & \textbf{23.31}                     \\\cmidrule{1-6}
                                                                            %  & FiD (open-book)  &    25.06         &     5.98        &       22.12      &  18.48   &  80.96   &   28.06            &     16.96                \\ \midrule
\multirow{3}{*}{WoW}                                                         & BART-Large                   &     \textbf{17.22}        & 15.37   & 11.78               & 4.05                       \\
                                                                             & EDMem-free     &               16.52           & 15.28     & 16.71              & 6.83                       \\
                                                                             & EDMem-dyn.          &     17.01             & \textbf{15.51}     & \textbf{17.29}             & \textbf{7.81}   \\
                                                                            %  & FiD (open-book)  &      22.72       &      6.43       &        20.16     &  18.48   &   81.06  &   17.91            &     11.99                \\ 
                                                                             \bottomrule
\end{tabular}}
\caption{Results on entity-intensive generation datasets. \textbf{Bold} scores are best results among closed-book models.}
\label{tab:geneartion}
% \vspace{-0.1cm}
\end{table*}

==> tables/table-hyper_QA.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.3mm}{
\resizebox{0.48\textwidth}{!}{\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{\textbf{Hyper-Parameter}} & \multicolumn{2}{c}{\textbf{TQA}} & \textbf{NQ}    & \textbf{WQ}    \\
                                & In-House Test   & Dev   & Test           & Test           \\  \midrule
Learning Rate        & 5e-6 & 1e-5 & 3e-5 & 2e-5 \\
$\lambda_{EL}$         & 1.0 & 1.0  & 1.0  & 0.5  \\
Dropout Rate         & 0.1 & 0.1  & 0.2  & 0.1  \\
Batch Size           & 256 & 256 & 256  & 128  \\
Training Steps       & 19K & 13K & 21K  & 2K \\
Beam Size            & 1  &  1 & 1    & 1    \\
\#Candidate Entities & 1 &  1  & 1    & 1   \\
Validation Perform. & 40.77 & 43.32 & 28.53 & 38.89\\ \bottomrule
\end{tabular}}}
\caption{Hyper-parameters used in fine-tuning on open-domain QA datasets. ``\#Candidate Entities'' is the number of candidate entities in constrained entity generation. ``Validation Perform.'' is the EM score on dev set under the setting of free-form generation.}
\label{tab:hyper_qa}
\end{table}

==> tables/table-hyper_gen.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1mm}{
\resizebox{0.48\textwidth}{!}{\begin{tabular}{l|cccc}
\toprule
\textbf{Hyper-Parameter} & \textbf{MSMARCO} & \textbf{CREAK} & \textbf{ELI5} & \textbf{WoW} \\ \midrule
Learning Rate            & 5e-6             & 1e-5           & 1e-5          & 1e-5         \\
$\lambda_{EL}$           & 0.5              & 2.0            & 0.5           & 0.5          \\
Dropout Rate             & 0.1              & 0.1            & 0.3           & 0.1          \\
Batch Size               & 256              & 128            & 128           & 128          \\
Training Steps           & 28K              & 1.8K           & 7.2K          & 6K           \\
Beam Size                & 5                & 5              & 5             & 5            \\
\#Candidate Entities     & 5                & 5              & 1             & 5       \\
Validation Perform. & 56.41 & 37.33 & 17.96 & 15.98
\\ \bottomrule
\end{tabular}}}
\caption{Hyper-parameters used in fine-tuning on generation datasets. ``\#Candidate Entities'' is the number of candidate entities in constrained entity generation. ``Validation Perform.'' is the validation score (WoW: F1, others: ROUGE-L) on dev set under the setting of free-form generation.}
\label{tab:hyper_gen}
\vspace{-0.2cm}
\end{table}

==> tables/table-linkable-demo.tex <==

\begin{table*}[t]
\centering
\setlength{\tabcolsep}{1.3mm}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\multicolumn{1}{l|}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{3}{c|}{\textbf{TQA}}                                                                            & \multicolumn{3}{c|}{\textbf{NQ}}                           & \multicolumn{3}{c}{\textbf{WQ}}                          \\
\multicolumn{1}{c|}{}                           & \multicolumn{3}{c|}{Official Dev}                 & \multicolumn{3}{c|}{Test}                         & \multicolumn{3}{c}{Test}                        \\
                                           & Total          & Ent.       & Non-Ent.   & Total          & Ent.       & Non-Ent.   & Total          & Ent.       & Non-Ent.  \\ \midrule
BART                                               & 27.28            &  30.52           & 9.70           & 24.82          & 28.54          & 15.95          & 29.23          & 32.28          & 5.24          \\
EaE                                              & 43.20          & 51.43          & 0.00           & -              & -              & -              & 39.00          & 42.86          & 0.00          \\
EncMem                                        & 42.00          & 49.74          & 0.00           & 25.54          &  36.24 & 0.00           &   38.88   &   43.82  & 0.00          \\
EDMem-free                                & 43.31          & 49.44          & \textbf{10.10} & 29.14          & 34.32          & \textbf{16.19} & 36.47          & 40.16          & \textbf{7.42} \\
EDMem-stat.                                     & \textbf{47.23} & \textbf{54.86} & 5.85           & \textbf{30.19} & \textbf{37.38}          & 13.04          & \textbf{41.44}          & \textbf{46.26}          & 3.49          \\
EDMem-dyn.                                  & 44.44          & 51.10          & 8.29           & 27.70          & 33.41          & 14.07          & 39.52          & 44.09          & 3.49          \\ \bottomrule
\end{tabular}}}
\caption{Exact match scores on entity answers (``Ent.'') and non-entity answers (``Non-Ent.'') in open-domain QA.}
\label{tab:linkable}
% \vspace{-0.1cm}
\end{table*}    
